On statistic alignment for domain adaptation in structural health monitoring

The practical application of structural health monitoring (SHM) is often limited by the availability of labelled data. Transfer learning - specifically in the form of domain adaptation (DA) - gives rise to the possibility of leveraging information from a population of physical or numerical structures, by inferring a mapping that aligns the feature spaces. Typical DA methods rely on nonparametric distance metrics, which require sufficient data to perform density estimation. In addition, these methods can be prone to performance degradation under class imbalance. To address these issues, statistic alignment (SA) is discussed, with a demonstration of how these methods can be made robust to class imbalance, including a special case of class imbalance called a partial DA scenario. SA is demonstrated to facilitate damage localisation with no target labels in a numerical case study, outperforming other state-of-the-art DA methods. It is then shown to be capable of aligning the feature spaces of a real heterogeneous population, the Z24 and KW51 bridges, with only 220 samples used from the KW51 bridge. Finally, in scenarios where more complex mappings are required for knowledge transfer, SA is shown to be a vital pre-processing tool, increasing the performance of established DA methods.

==> defin.tex <==
\section{Domain Adaptation}
In this section, the domain adaptation problem in PBSHM is outlined. Before defining domain adaptation formally, it is necessary to provide some relevant definitions \cite{Weiss2016}\cite{Pan2010a},\\

\noindent\textbf{Definition 2}: A \emph{domain} $\mathcal{D}=\{\chi,p(X)\}$, is defined by a feature space $\chi$ and marginal distribution $P(X)$, where $X=\{\mathbf{x}_1,...,\mathbf{x}_n\} \in \chi$.\\
\textbf{Definition 3}: Given a domain, a \emph{task} $T=\{\mathcal{Y},f(.)\}$, is defined by a label space $\mathcal{Y}$ and, a predictive function $f(.)$, learnt from training data $\{X,\mathbf{y}\}$, where $\mathbf{y}\in \mathcal{Y}$. \\\\
Thus, transfer learning can be defined as:\\\\
\textbf{Definition 4}: For a given source domain $\mathcal{D}_s$ and task $T_s$; target domain $\mathcal{D}_t$ and task $T_t$, \emph{transfer learning} is the process of improving the performance of $f_t(.)$ in $T_t$, using domain invariant information learnt from $\mathcal{D}_s$ and $T_s$. It is assumed $\mathcal{D}_s \neq \mathcal{D}_t$ and $T_s = T_t$ in homogeneous transfer learning. Heterogeneous transfer learning (which is not considered in this work) also assumes $T_s \neq T_t$.\\

\noindent As previously mentioned, domain adaptation is a particularly promising sub-field of transfer learning for PBSHM, defined as:\\\\
\textbf{Definition 5}: \emph{Domain adaption} is a category of transfer learning, assuming disparity between the marginal distributions $P(X_s) \neq P(X_t)$, and/or the conditional distributions $P(Y_s|X_s) \neq P(Y_t|X_t)$. The approach attempts to transform one or more source domains $\mathcal{D}_s$ and a target domain $\mathcal{D}_t$, to a domain-invariant space that minimises distribution discrepancy. As such, a classifier trained either entirely, or partly on the source will generalise to the target domain.\\

\noindent A major challenge in unsupervised or semi-supervised DA is that, without label information, reliable validation via estimation of the empirical risk is not possible. As such poor classification should be avoided by robust transfer learning approaches:  \\\\

\textbf{Definition 6}: If a transfer learner achieves worse classification than would be obtained by using target label data (if there is any) or a source classifier to classify target instances, \emph{negative transfer} has occurred. \\

%show classification can be done with just normal -> class 1 -> etc
%fully adapting correlation of a sparse normal condition is unreliable
\noindent PBSHM aims to alleviate the requirement of damage-state labels by leveraging labels from similar structures, $\{X_{s},\mathbf{y}_{s}\}$. Initially, the target structure would consist of only a limited amount of normal condition data, then would accumulate data for a wider range of operating conditions, damage-state data and, after repair, corresponding labels. At first, adaptation is limited to adapting the statistics of the normal condition. In doing so, a novelty detector may be improved or, as is demonstrated in this work, even damage localisation may be attempted. As class information in the target structure becomes available, the distributions could be further harmonised using DA.\\

It is clear that, to perform damage localisation, the source must be populated with damage-state data. However, determining what subset of damage-states are most appropriate to transfer is not trivial. Thus, the source domain(s) must contain examples for each damage-location of interest. This issue will cause sample bias, whereby a bias is caused because the probability of sampling features across the feature space is inconsistent \cite{Sugiyama2008}.   This motivates framing the PBSHM problem as a partial domain adaptation problem:\\\\

\textbf{Definition 7}: \emph{Partial domain adaption}  is a special case of domain adaption where the target domain contains data pertaining to fewer classes than the source, $\mathcal{Y}_t\subseteq \mathcal{Y}_s$. \\

In PBSHM, there are a numerous applications for which domain adaptation could be applied. Previous work has also looked at unsupervised domain adaptation for damage localisation \cite{Gardner2020}, account for changes in distributions induced by repair \cite{Gardner2021}, as well as damage detection and quantification \cite{Xu2020}. These works consider unsupervised DA. This report considers this case, as well as, unsupervised partial DA.\\

%there is a problem with this?




\subsection{Distribution Distance Metrics}
%explain median heuristic
There are a number of approaches to DA \cite{Weiss2016}, perhaps one of the most common is minimising a metric that corresponds to difference between the distributions. A distance metric can be used to test whether $X_s$ and $X_t$ have been sampled from the same distribution, whereby $d(P(X_s),P(X_t))$=0 only if $P(X_s)=P(X_t)$, where $d(P(X_s),P(X_t))$ is some distance metric between the probability distributions $P(X_s)$ and $P(X_t)$. One such metric is the \emph{Maximum Mean Discrepancy (MMD)} \cite{Gretton2012}.  A kernel map $\phi$, is utilised to embed the original feature in a Reproducing Kernel Hilbert Space (RKHS), $\phi: X \rightarrow H$. The empirical estimate of the (squared) MMD can be defined by,
\begin{equation}
    MMD(P(X_s),P(X_t))=\| \frac{1}{n_s}\sum_{i=1}^{n_s}\phi (\mathbf{x}_{s,i})-\frac{1}{n_t}\sum_{i=1}^{n_t}\phi (\mathbf{x}_{t,i})  \|^2_H
\end{equation}
The MMD is therefore the difference between the mean of the kernel embeddings of each domain. \\
%lit review here?

%define A-distance
%intuitively A-distance is the biggest differnece in classification probability within a set of data of interest
%cannot be estimated though 
%PAD
%not a relevant bound but 
%useful for reasoning about transfer and explain similarities to GANs

%then later put the bound in short

%define H-divergence then proxy A
Another distance metric that can provide valuable insight into how transferable domains are is the $\mathcal{H}$-divergence \cite{Ben-David2007}. Given  the probability distributions $P(X_s)$ and $P(X_t)$ over the feature space $\chi$ and hypothesis class $h\in \mathcal{H}$ the  $\mathcal{H}$-divergence is defined as,
\begin{equation}
    d_\mathcal{H}(P(X_s),P(X_t))=2 \underset{h\in H}{\sup} | Pr(h(\mathbf{x}_s)=1) -Pr(h(\mathbf{x}_t)=1)| 
\end{equation}  
Intuitively, this states the similarity between the marginal probability distributions can be measured by the largest difference in prediction probability of a classifier $f()$, within a set of interest. The hypothesis class $\mathcal{H}$, has bounded capacity (VC dimension) and is sufficiently rich that it can achieve low error in both domains. \\

%A distance no H distance
Directly computing $\mathcal{H}$-divergence directly isn't feasible, as it would require exhaustively evaluating $h\in \mathcal{H}$. Ben-David \emph{et al.} \cite{Ben-David2007} suggest training a domain discriminator is equivalent to Equation 1.24. The error $\epsilon$ can then be used to approximate $\mathcal{H}$ divergence,
\begin{equation}
    \hat{d}_\mathcal{A}=2(1-2\underset{h\in\mathcal{H}}{min}(\epsilon))
\end{equation}
 As is standard practice, optimisation is performed on a convex upper-bound of the classifier error. Therefore, this approach provides an \emph{estimation} of $\mathcal{H}$-divergence, named the Proxy- $\mathcal{A}$-distance (PAD).\\ %confusing

A number of other metrics have been used in DA, Kullback-Leibler (KL) Divergence \cite{Dai2007}, Jensen-Shannon Divergence \cite{Chen2010}, Bregman Divergence\cite{Si2010}, Hilbert-Schmidt Independence Criterion\cite{Wang2011}\cite{Yan2017}, to name a few. 
 
\subsection{Transfer Component Analysis}
Transfer component analysis (TCA), can be seen as an extension to kernelised PCA, that aims to find axis that maximises variance and minimises the MMD.  TCA makes the assumption that $P(X_s) \neq P(X_t)$ but the kernel mapping found $\phi$, preserves discriminative information, satisfying $P(Y_s |\phi(X_s)) \approx P(Y_t|\phi(X_t))$ \cite{JialinPan2011}.  However, because of unavailability of target labels, the MMD used to find $\phi$ is only minimising distance between marginal distributions; the assumption $P(Y_s |\phi (X_s)) \approx P(Y_t|\phi (X_t))$ will break down under high conditional distribution discrepancy, potentially causing negative transfer.  The problem can then be formulated as an optimisation problem for the transformation matrix $A$ (details can be found in appendix A.3),
\begin{equation}
    \underset{A^TKHKA=I}{min}tr(A^TKMKA)+\lambda tr(A^TA)
\end{equation}
where $tr()$ are the diagonal elements of the matrix, $M$ is the MMD matrix, $K$ is the kernel matrix, $H$ is a centring matrix $H=I-\frac{1}{n_s+n_t}\mathbf{1}$, and $\mathbf{1}$ is a matrix of ones. Optimisation is carried out with the regularisation restraint $tr(A^TA)$, controlling complexity of $W$, scaled by $\lambda$ and is subject to a kernel PCA constraint, $A^TKHKA=I$, to preserve discriminative information and prevent the trivial solution of driving $A$ to zero. If only MMD was minimised a noisy component with no useful domain specific information could be selected. 

\subsection{Joint Distribution Adaptation}
Joint distribution adaptation (JDA) \cite{Long2013} extends TCA to address the case $P(Y_s |\phi(X_s)) \ne P(Y_t|\phi(X_t))$. To alleviate the limitations in adapting the conditional distributions without target labels, JDA utilises pseudo-labels, $\hat{\mathbf{y}}_{t,pseudo}$. Furthermore, the posterior distributions $P(Y|X)$ are difficult to estimate, so JDA uses the class-conditional probabilities $P(X|Y)$. To do so it measures the MMD between samples belonging a a single class such that, 
\begin{equation}
    \underset{A^TKHKA=I}{min}tr(A^TK\sum_{c=0}^{C}M_cKA)+\lambda tr(A^TA)
\end{equation}
where $M_c$ is the MMD between data in class c $c\in \mathcal{Y}$ (see appendix A.4), and $c=0$ is the original MMD matrix; to overcome the lack of labels in the target domain, a classifier trained on transformed space is used to predict pseudo-labels $\hat{y}_{t,pseudo}$. To find accurate target labels, a number of iterations are required \cite{Long2013}. 

\subsection{Geodesic Flow Kernel}

In contrast to the previous kernel methods that minimise a distance measure, the geodesic flow kernel (GFK) utilises the assumption that a geodesic flow, existing on a Grassmannian  manifold, exists between the PCA subspaces of the source and target \cite{Gong2012}. A geodesic flow is a smooth curve that gives the shortest path between two points on a Riemannian manifold, in this case the source and target subspaces. The method is then to find a projection of all the subspaces along the geodesic curve, utilising the kernel trick. The approach also offers a way to select the most similar subspaces, by the subspace disagreement measure (SDM) \cite{Gong2012}. As such the approach can be summarised as: finding the optimal subspaces by comparing (SDM), constructing the geodesic curve, computing the geodesic flow kernel, and building a classifier using the kernel features. Details can be found in appendix A.5.
%this is just an overview derivations found in supplementary


\subsection{Domain Adversarial Neural Network}
Following the success of the generative adversarial network (GAN) \cite{Goodfellow2014}, the DANN attempts to incorporate the two-player game approach into a DA regularisation term \cite{Ganin2017}. It is an example of an \emph{adversarial approach} to deep DA \cite{Zhuang2021}.\\

The architecture of the domain adversarial neural network (DANN) can be found in figure \ref{fig:DANN}. A feature extractor $G_f()$, finds a domain invariant space by simultaneously being trained to classify the source samples $G_y()$, and to fool a domain discriminator $G_d()$.
\begin{figure}[h!]
\centering
\includegraphics[width=12cm]{DANN.png}
\caption{DANN architecture \cite{Ho2002}}
\label{fig:DANN}
\end{figure}

During training source and target samples are fed into the network as pairs. Both are transformed via the feature extractor, then the source classifier predicts the label for the source instance, and the domain discriminator attempts to label the domain of each instance. The gradient between the feature extractor and domain discriminator is reversed, utilising a novel gradient reversal layer \cite{Ho2002}, so the feature space attempts to fool the domain discriminator. Hence, features are found that minimise the PAD and maximise discriminative information. Details of the loss function and gradient reversal layer can be found in appendix A.6.

\subsubsection{Mode Collapse}
Training of GANs is notoriously difficult \cite{Mescheder2018}. A common issue is mode collapse, where multiple classes are mapped to one class, in an attempt to trick the discriminator, depicted in Figure \ref{fig:collapse}. This is a sub-optimal solution that is also found in the adversarial DA approaches. 

\begin{figure}[h!]
\centering
\includegraphics[width=6cm]{mode collapse.png}
\caption{An example of mode collapse. Class 1 and 2 in the target (in orange), have both been mapped to class 2 in the source (in blue).}
\label{fig:collapse}
\end{figure}
\subsection{Distribution Estimation in Plots}
An estimation of the marginal distributions are visualised in each plot in this work, as seen at the top and right of Figure \ref{fig:collapse}. These are found via kernel density estimation (KDE), utilising an RBF kernel (see \cite{Murphy2014} for details). 

\subsection{Normalisation in Transfer Learning}
For knowledge transfer, normalisation can minimise discrepancy between the marginal distributions, by adapting the first two sufficient statistics mean $\mu$, and standard deviation $\sigma$. In deep DA, adapting these statistics has shown to improve speed of convergence and overall classification by utilising variations of domain specific BN \cite{Li2018}\cite{Chang2019}\cite{Seo2020}. This differs to traditional normalisation they aim to overcome \emph{internal} covariate shift. \\
Another approach with similarities to normalisation is Euclidean alignment (EA) \cite{He2020}. It aligns the mean of entire correlation matrices from multiple EEG signals, and suggests using the aligned correlation matrices as features. A similar approach CORAL \cite{Sun2016}, whitens the source (centres and decorrelates the features), then "recolours" such that the source features are re-correlated by the target correlation. These are \emph{statistic feature-alignment} approaches to DA, defined by:\\

\textbf{Definition 8}: \emph{Statistic-feature alignment} is an approach to DA that aims to adapt the domains by aligning one or more of their statistics, commonly the mean, standard deviation or correlation \cite{Zhuang2021}.\\

Normalisation has been shown to improve the performance of TCA in software detection Nam et al. \cite{Nam2013}. The work defines a strategy for normalisation for TCA based on euclidean pairwise distances within each domain. The proposed methods include, min-max normalisation, standardisation, as well as two variants of standardisation defined as,
\begin{equation}
\begin{aligned}
     \mathbf{z}_s^{(j)}=\frac{\mathbf{x}_s^{(j)}-\mu_{s,j} }{\sigma_{s,j}}\\
    \mathbf{z}_t^{(j)}=\frac{\mathbf{x}_t^{(j)}-\mu_{s,j} }{\sigma_{s,j}}
\end{aligned}
\end{equation}

\begin{equation}
\begin{aligned}
     \mathbf{z}_s^{(j)}=\frac{\mathbf{x}_s^{(j)}-\mu_{t,j} }{\sigma_{t,j}}\\
    \mathbf{z}_t^{(j)}=\frac{\mathbf{x}_t^{(j)}-\mu_{t,j} }{\sigma_{t,j}}
\end{aligned}
\end{equation}
These methods are suggested for the case that data one domain are sparse or dense, such that estimation of the sufficient statistics would be inaccurate.

\subsection{Statistical Alignment by Standardisation for PBSHM}

This report considers any normalisation that reduces the discrepancy between the means and/ or the standard deviations (more generally the scale), as a DA approach, specifically statistic-feature alignment. A common assumption in novelty detection is that, data collected at the start of a structures operation can be assumed to have come from the normal condition \cite{Dervilis2015}. Under this assumption, it is proposed normalisation can be performed in a way that aligns the normal conditions, called \emph{normal-standardisation},
\begin{equation}
\begin{aligned}
    \mathbf{z}_s^{(j)}=\frac{\mathbf{x}_s^{(j)}-\mu_{s,j}}{\sigma_{s,j}}\\ \mathbf{z}_t^{(j)}= \frac{\mathbf{x}_t^{(j)}-\mu_{t,j}}{\sigma_t}-(\mu_{t,\textrm{normal},j}-\mu_{s,\textrm{normal},j})
\end{aligned}
\end{equation}
%perhaps comparing this to mean matching but no scaling?
where $\mu^{(j)}_{s,normal,j}$ and $\mu^{(j)}_{t,normal,j}$ are the means of the normal condition for feature $j$, of the source and target respectively . Standardising in this way, avoids the assumption that by aligning the mean of the entire domain, the classes will be well aligned, which may not be the case when the conditional distributions differ, an example of this is shown in Section 1.5. Instead, at least the normal condition will be correctly aligned, and it is hypothesised that the transfer learner will seek to find a domain invariant representation that maintains $P(X_{s,normal})\approx P(X_{t,normal})$.  \\

In addition, in partial DA, damage-state features are not available for all classes in the target. This means, estimating the mean and standard deviation of the entire domain is not possible, potentially causing domains to be incorrectly aligned if normalised with a standard approach, which was illustrated in Figure \ref{fig:gen approach} . To perform standardisation in this scenario, \emph{Partial-Standardisation} is proposed,
\begin{equation}
\begin{aligned}
 \mathbf{z}_s^{(j)}=\frac{\mathbf{x}_s^{(j)}-\mu_{s,j}}{\sigma_{s,j}}\\ \mathbf{z}_t^{(j)}= \frac{\sigma_{s,\textrm{normal},j}}{\sigma_{t,\textrm{normal},j}}(\mathbf{x}_t^{(j)}-\mu_{t,j})-(\mu_{t,\textrm{normal},j}-\mu_{s,\textrm{normal},j})
\end{aligned}
\end{equation}
where $\sigma_{s,normal,j}$ and $\sigma_{t,normal,j}$ are the standard deviations of the source and target normal condition data for $j^{th}$ feature. This method allows the mean distance to be minimised, shown in Figure \ref{fig:normnorm} a). However, if it is assumed the initial spaces are similar, scaling the source domain, and not the target would cause a large disparity in the scales. Another possibility is that causes of increased variation in the standard deviation in one domain $\sigma_s\not\approx\sigma_t$, may be reflected by an increase in standard deviation of their classes $\sigma_{s,normal}\not\approx\sigma_{t,normal}$. In both of these cases aligning the standard deviation of the normal conditions $\sigma_{s,normal}=\sigma_{t,normal}$, would also align the standard deviations $\sigma_s\approx\sigma_t$, shown in Figure \ref{fig:normnorm} b). The adaptation of scale may not be exact, but as suggested in the following section, approximately matching it may be sufficient. 

\begin{figure}[H]%BAD EXAMPLE CHANGE
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{mean align.png}
         \caption{ }
         \label{fig:bad norm}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{PBSHM.png} 
         \caption{ }
         \label{fig:cool sping }
     \end{subfigure}
     \caption{ Demonstration of aligning the normal condition means in a), and then normal condition standard deviations in b).}
     \label{fig:normnorm}
\end{figure}



%coutner intuitive when considering target is similar to a test dataset whereby stanard practice dictates the same procedure should be applied to all 
